JIZHI: A Fast and Cost-Effective Model-As-A-Service System for Web-Scale Online Inference at Baidu

In modern internet industries, deep learning based recommender systems have became an indispensable building block for a wide spectrum of applications, such as search engine, news feed, and short video clips. However, it remains challenging to carry the well-trained deep models for online real-time inference serving, with respect to the time-varying web-scale traffics from billions of users, in a cost-effective manner. In this work, we present JIZHI - a Model-as-a-Service system - that per second handles hundreds of millions of online inference requests to huge deep models with more than trillions of sparse parameters, for over twenty real-time recommendation services at Baidu, Inc. In JIZHI, the inference workflow of every recommendation request is transformed to a Staged Event-Driven Pipeline (SEDP), where each node in the pipeline refers to a staged computation or I/O intensive task processor. With traffics of real-time inference requests arrived, each modularized processor can be run in a fully asynchronized way and managed separately. Besides, JIZHI introduces heterogeneous and hierarchical storage to further accelerate the online inference process by reducing unnecessary computations and potential data access latency induced by ultra-sparse model parameters. Moreover, an intelligent resource manager has been deployed to maximize the throughput of JIZHI over the shared infrastructure by searching the optimal resource allocation plan from historical logs and fine-tuning the load shedding policies over intermediate system feedback. Extensive experiments have been done to demonstrate the advantages of JIZHI from the perspectives of end-to-end service latency, system-wide throughput, and resource consumption. JIZHI has helped Baidu saved more than ten million US dollars in hardware and utility costs while handling 200% more traffics without sacrificing inference efficiency.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle


==> exp.tex <==
\section{Experimental evaluation}\label{sec:exp}

\subsection{Experimental Setup}
In this section, we conduct extensive experiments to evaluate the effectiveness of the proposed system.
We report evaluations on four different \spred empowered real-world online inference services deployed in Baidu. All results are collected from the online living system.
Specifically, \emph{Service A} is for a multi-modal recommendation model on Baidu news feed, \emph{Service B} and \emph{Service C} are video recommendation services used in different product scenarios, \emph{Service D} is a multi-objective recommendation service fulfilling multiple targets.
%\emph{Model E} is a ranking model used in Baidu search engine, 
\tabref{table-data} summarizes model statistics of five recommendation services.
We use the previous online inference system~(\legacy) as described in \secref{sec:back} as the compared baseline.

\begin{table}[t]
\centering
%\begin{footnotesize}
%\vspace{-6ex}
\caption{Statistics of online inference services.}
\vspace{-3ex}
\begin{tabular}{c | c c c} \hline
& Model size & \# of feature groups & Traffic load\\ \hline\hline
Service A & 430 GB & 379 & $4.58\times 10^8/s$ \\
Service B & 500 GB & 430 & $4.21\times 10^8/s$ \\
Service C & 285 GB & 270 & $3.67\times 10^7/s$ \\
Service D & 210 GB & 106 & $7.15\times 10^7/s$ \\
%Model E & 70 & 134 & XX \\
%Service E & 1,743 GB & 968 & 91.98 million \\
\hline
\end{tabular}
%\end{footnotesize}
\label{table-data}
\vspace{-3ex}
\end{table}

In the evaluation, we focus on system performance metrics. We use latency, throughput, and the number of required instances~(\ie the computational resource) to evaluate the efficiency and cost-effectiveness of the system. Specifically, the latency is computed as the averaged time per task~(user-item pair) in millisecond~(ms), the throughput is defined as the number of tasks processed per second.
An instance refers to a virtual machine on the cloud, which is commonly equipped with four CPU cores, 20 GB memory, and shares 8 TB disk in a physical server~(4TB SSD and 4TB SATA).

\subsection{Overall Production Experience}
\tabref{table-result} reports the overall performance of \spred compared with the legacy online inference system on four different services with respect to three metrics. 
As can be seen, \spred outperforms \legacy on all services in terms of all metrics. Specifically, \spred achieves (23.33\%, 17.24\%, 2.5\%, 18.18\%) latency improvement and (188.37\%, 178.13\%, 86.16\%, 133.41\%) throughput improvement on four services, respectively. Benefit from such improvement, \spred reduces (65.33\%, 62.56\%, 46.3\%, 57.17\%) instances in the online serving infrastructure without sacrificing system efficiency, which helps Baidu save over ten million US dollars' computational resource budgets~(hardware, energy consumption, labor cost, \etc) per year. And we foresee this economic gain will improve with the future traffic load growth of each recommendation service.
Further look into the performance of each service, we notice the performance gain of Service C is relatively lower than others, which mainly because the corresponding product is resource constrained~(\ie less budget than others), and the system is tuned to minimize the resource consumption.
%workflow is simple, and \TODO{XX}, with left less optimization space in online inference.

\begin{table}[t]
\centering
%\begin{footnotesize}
%\vspace{-6ex}
\caption{Overall performance.}
\vspace{-3ex}
\begin{tabular}{c |c| c c c c} \hline
\multicolumn{2}{c|}{}  & Latency & Throughput & \# of instance \\ \hline \hline
\multirow{2}{*}{Service A} & \legacy & 30 ms & $1.53\times 10^6$ & 11,450 \\
                         & \spred & 23 ms & $4.42\times 10^6$ & 3,970 \\
                         %& Gain   & 23.33\% & 188.37\% & 65.33\% \\\hline
\multirow{2}{*}{Service B} & \legacy & 29 ms & $1.63\times 10^6$ & 12,750 \\
                         & \spred & 24 ms & $4.36\times 10^6$ & 4,773 \\
                         %& Gain   & 17.24\% & 178.13\% & 62.56\% \\\hline
\multirow{2}{*}{Service C} & \legacy & 41 ms & $2.8\times 10^6$ & 2,067 \\
                         & \spred & 40 ms & $5.21\times 10^6$ & 1,110 \\
                         %& Gain   & 2.5\% & 86.16\% & 46.3\% \\\hline
\multirow{2}{*}{Service D} & \legacy & 22 ms & $3.53\times 10^6$ & 4280 \\
                         & \spred & 18 ms & $8.24\times 10^6$ & 1833 \\\hline
                         %& Gain   & 18.18\% & 133.41\% & 57.17\%\\\hline
\end{tabular}
%\end{footnotesize}
\label{table-result}
\vspace{-4ex}
\end{table}

\subsection{Effect of SEDP}
Then we look into the inference time distribution to study the effect of SEDP. Due to page limit, we only report the results on Service A, the results on other services are similar.
%We calculate the latency and traffic load for each recommendation service by collecting one week online logs, ranged from 2021, January 24 to 2020, January 30.
\begin{figure}[t]
    %\vspace{-3ex}
	\begin{minipage}{1.\linewidth}
    \centering
    \subfigure[Latency distribution.]{
        \includegraphics[width=.45\linewidth]{KDD21-JIZHI/figs/latency_cdf.pdf}
        \label{fig:latency-dist}
    }
    \subfigure[Latency v.s. traffic.]{
        \includegraphics[width=.45\linewidth]{KDD21-JIZHI/figs/latency_traffic.pdf}
        \label{fig:latency-traffic}
    }
    \subfigure[Latency breakdown by hour.]{
        \includegraphics[width=.45\linewidth]{KDD21-JIZHI/figs/stacked_latency_hour.pdf}
        \label{fig:stack-latency-hour}
    }
    \subfigure[Latency breakdown by traffic.]{
        \includegraphics[width=.45\linewidth]{KDD21-JIZHI/figs/stacked_latency_traffic.pdf}
        \label{fig:stack-latency-traffic}
    }
    \end{minipage}
    \vspace{-4ex}
    \caption{Effect of SEDP on latency.}
    \vspace{-5ex}
    \label{fig:latency}
\end{figure}

We first study the overall latency distribution.
\figref{fig:latency-dist} and \figref{fig:latency-traffic} report the overall online inference latency distribution and the latency distribution with respect to the varying traffic load, respectively.
As can be seen, the overall latency follows a bimodal distribution. This makes sense as the first peak corresponds to requests hit two caches, and the second peak corresponds to majority requests in the peak hour.
Moreover, we observe the latency increases sub-linearly with respect to the traffic load growth, which verifies the robustness of the system under time-varying traffics.

\figref{fig:stack-latency-hour} and \figref{fig:stack-latency-traffic} breakdown the latency into four major stages, \ie user related processing, item related processing, cube related processing, and DNN forward computation. 
%Based on the recommendation logic of Service A, we break the latency into four major inference stages.
Overall, we observe the ratio of latency in each stage is relatively stable at different hours and traffic loads.
Moreover, the overall latency slightly increases in the evening peak hour.
Besides, with the traffic load growth, we observe the averaged latency first decrease and then increase. This is related to the cache hit ratio, which first increases when the ratio of frequent requests increase and then decreases when more long-tailed items flush two caches. 

\subsection{Effect of the Storage Module}\label{sec:exp-cache}
We report the hit ratio of the cube cache and the query cache at different hours of Service A in a whole week to demonstrate the effect of the heterogeneous and hierarchical storage, as shown in \figref{fig:cache}. 
Overall, the hit ratio of two caches are varying by hour and showing strong daily periodicity, which is highly correlated with the traffic load variation.
In particular, the cube cache achieves $84.21\%$ hit ratio in average and the daily variation is less than $3.61\%$, while the query cache yield $19.26\%$ hit ratio in average but with a higher variation range.
In summary, the cube cache achieves higher hit ratio and every hit reduces partial data access latency, while the query cache achieves a relative lower hit ratio but per hit eliminates the whole inference task computation.
Two caches are robust to reduce the inference latency and computational overhead at different times in the week.

\begin{figure}[t]
    \centering
    %\vspace{-10ex}
    \includegraphics[width=.45\textwidth]{KDD21-JIZHI/figs/cache_hit.pdf}
    \vspace{-15pt}
    \caption{Hit ratio of the cube cache and query cache.}
    \vspace{-10pt}
    \label{fig:cache}
\end{figure}

\begin{figure}[t]
    \centering
    %\vspace{-3ex}
    \includegraphics[width=.45\textwidth]{KDD21-JIZHI/figs/cutoff.pdf}
    \vspace{-15pt}
    \caption{Cutoff ratio in Service A.}
    \vspace{-10pt}
    \label{fig:cutoff}
\end{figure}

\subsection{Effect of the Intelligent Resource Manager}
We further justify the performance gain of 
%the intelligent resource manager, including 
the offline resource optimization and online load shedding.

\textbf{Offline resource optimization}.
\tabref{table-offline-opt-gain} reports the quantitative results of the resource gain of each service with the offline resource optimization. 
%Note that the primary objective of offline auto-tuning is to reduce computational resources. The optimization is with the constraint of keep latency unchanged.
As can be seen, the offline resource optimization module successfully reduces $8.91\%$ to $16.45\%$ instances without sacrificing system latency.
We further conduct the qualitative study by comparing key optimization parameters of Service A before~(\emph{noOpt}) and after~(\emph{Opt}) applying offline resource optimization, which is shown in \tabref{table-offline-opt-case}. As can be seen, the resource manager assigns a larger batch size to most stage processors except the cube accessor. This makes sense since over $80\%$ computations in this stage is reduced by the cube cache, as discussed in \secref{sec:exp-cache}.
Moreover, the size of the cube cache and the expire window of the query cache are increased, and the offline manager derives a more aggressive memory allocation strategy. Such settings can further reduce the data access latency and improve the CPU utilization, which therefore improves the overall resource utilization rate.

\begin{table}[t]
\centering
%\begin{footnotesize}
%\vspace{-2ex}
\caption{Resource gain of offline auto-tuning.}
\vspace{-3ex}
\begin{tabular}{c| c c} \hline
Service & Reduced \# of instance & Gain \\ \hline \hline
A & 1,636 & 14.29\% \\
B & 1,736& 13.62\%\\
C & 184 & 8.91\% \\
D & 704 & 16.45\%\\\hline
\end{tabular}
%\end{footnotesize}
\label{table-offline-opt-gain}
\vspace{-2ex}
\end{table}

\begin{table}[t]
\centering
%\begin{footnotesize}
%\vspace{-8ex}
\caption{Offline auto-tuning results in Service A.}
\vspace{-3ex}
\begin{tabular}{c c| c | c} \hline
Category & Parameter & \emph{noOpt} & \emph{Opt} \\ \hline \hline
\multirow{5}{*}{Stage} & User batch & 30 & 34 \\
 & Item extractor batch & 4 & 12 \\
 & Item processor batch & 6 & 17 \\
 & Cube batch size & 10 & 6 \\
 & DNN batch size & 15 & 25 \\\hline
\multirow{5}{*}{System} & Cube cache ratio & 1\% & 1.2\% \\
 & Query cache window & 120s & 143s \\
 & \# of arenas & 500 & 549 \\
% & Junk filling &  & False \\
 & Max active extent & 6 & 25 \\
 & Huge page & Default & Always\\\hline
\end{tabular}
%\end{footnotesize}
\label{table-offline-opt-case}
\vspace{-2ex}
\end{table}

\textbf{Online load shedding}.
To illustrate the effectiveness of online load shedding,
\figref{fig:cutoff} depicts the cutoff ratio of the online load shedding and the corresponding traffic loads over a week. 
We observe highly synchronized fluctuations of the cutoff ratio and the traffic load. Specifically, in the evening peak hour of traffic load, we observe the peak of cutoff ratio simultaneously.
Besides, we observe a relatively higher cutoff ratio at midnight, perhaps because of a lower click ratio in this period, indicating more items can be safely dropped without influencing recommendation effectiveness.

Overall, both offline and online resource management components successfully tune the online inference system to achieve better performance automatically.

\subsection{Multi-Tenant Serving}
Finally, we use \emph{Service E}, a recommendation service including multiple DNNs, to demonstrate the effectiveness of multi-tenant support in \spred. 
Specifically, \emph{Service E} including three different deep learning models, namely \emph{CTR}, \emph{FR}, \emph{CMT}, where each model corresponds to a different recommendation target.
The models are $1,743$ GB in total, involve 968 different feature groups, and the service handles $9.19\times 10^7$ traffics per second.
By deploying each different model as individual services, \tabref{table-multitenant} reports the latency, throughput and number of instances of each individual services compared with the multi-tenant based online inference on \spred.
Overall, we observe similar system latency by simultaneously executing three different models, indicating a linear speedup ratio of parallelization in \spred.
Moreover, \spred achieves $82.68\%$ throughput improvement comparing with the bottleneck model~(\ie \emph{CTR}).
Most importantly, by integrating three individual models into a unified online inference service, \spred saves $73.69\%$ instances in the cluster without losing efficiency.
\spred is even more cost-effective in the multi-tenant scenario than other single-model services~(\ie Service A to Service D).
This is because the unified service can reduce repetitive data access cost for multiple individual services~(\eg over $80\%$ feature groups are shared by three models), and largely reuses the intermediate results using the heterogeneous and hierarchical storage.

\begin{table}[t]
\centering
%\begin{footnotesize}
\caption{Effectiveness of multi-tenant serving.}
\vspace{-3ex}
\begin{tabular}{c| c c c} \hline
& Latency & Throughput & \# of instance \\ \hline \hline
\emph{CTR} & 50 ms & $2.48\times 10^6$ & 3,617 \\
\emph{FR} & 48 ms & $3.42\times 10^6$ & 2,560 \\
\emph{CMT} & 42 ms & $3.4\times 10^6$ & 1,350 \\\hline
\spred & 52 ms & $4.53\times 10^6$ & 1,980 \\\hline
%& Gain   & 18.18\% & 133.41\% & 57.17\%\\\hline
\end{tabular}
%\end{footnotesize}
\label{table-multitenant}
\vspace{-3ex}
\end{table}


